Siegel Brownian motion

We construct an analogue of Dyson Brownian motion in the Siegel half-space H that we term Siegel Brownian motion. Given \beta in (0,\infty], a stochastic flow for Z_t in H is introduced so that the law of the eigenvalues \lambda_t of the cross ratio matrix R(Z_t,iI_n) is determined by the Ito differential equation corresponds to stochastic gradient ascent of a function S. S turns out to be the log volume of isospectral orbit in H and can be understood as a Boltzmann entropy. In the limit \beta=\infty, the group orbits evolve by motion by minus a half times mean curvature.

==> results.tex <==
\section{Statement of results}
\label{sec:results}
Let $\bd B_t$ be the Brownian motion in $(\mathcal H,g)$, we propose the following SDE on $(\mathcal H,g)$, starting at $\bd Z_0$ with no repeated eigenvalues:
\begin{align}\label{sdeZ}
    \ud \bd Z_t=P_{Z_t}(\ud \bd B_t)+\sqrt{\frac2\beta}P^{\perp}_{Z_t}(\ud \bd B_t)
\end{align}
where $P_Z,P_Z^{\perp}$ are projection operators to the tangent space $T_Z\mathcal O_\lambda$ and its orthogonal complement $T_Z\mathcal O_\lambda^{\perp}$, where $\mathcal O_\lambda=G_{\ii I_n}\circ Z$ is  the $G_{\ii I_n}$ orbit of $Z$, $\lambda$ is the spectrum of $\mathfrak R(Z,\ii I_n)$ and $G_{\ii I_n}<\mathrm{Sp}(n,\mathbb R)$ is the stable subgroup of $\mathrm{Sp}(n,\mathbb R)$ fixing point $\ii I_n$. On Riemannian manifold the action of such projection operator on random processes is subtle, and will be discussed at the end of section \ref{sec3}.

The space downstairs $\Lambda$ is the space of spectrum of $\mathfrak R(Z,\ii I_n)$, and could be parametrized by the following:
\begin{align}
    \Lambda=&\{\text{eigenvalues of } (Z-\ii I_n)(Z+\ii I_n)^{-1}(\bar Z+\ii I_n)(\bar Z-\ii I_n)^{-1}|Z\in\mathcal H\}\nonumber\\
    =&\{\lambda=(\tanh^2{\frac{\sigma^1}2},...,\tanh^2{\frac{\sigma^n}2})|0\leq \sigma^1<\sigma^2<\cdots<\sigma^n, i=1,...,n\}
\end{align}

We have the following theorem describing the evolution of $\{\sigma^k(\bd Z_t)\}_{k=1}^n$.
\begin{theorem}\label{thm1}
    Let $\bd Z_t$ be a solution to SDE \ref{sdeZ}, $\lambda_t=(\tanh^2{\frac{\sigma_t^1}2},...,\tanh^2{\frac{\sigma_t^n}2})$ is the spectrum of $\mathfrak R(\bd Z_t,\ii I_n)$, then $(\sigma_t^1,...,\sigma_t^n)$solves the following SDE, in the sense that they have the same distribution
    \begin{align}\label{sdeSigma}
        \ud \sigma^k_t=&\frac12(\coth{\sigma^k_t}+\sum_{l\neq k}\frac{\sinh{\sigma^k_t}}{\cosh{\sigma^k_t}-\cosh{\sigma^l_t}})\ud t+\sqrt{\frac2\beta}\ud W^k_t&&k=1,...,n
    \end{align}
    where $\{W^k_t\}_{k=1}^n$ are $n$ independent Wiener processes.
\end{theorem}

Proof of theorem \ref{thm1} will be provided in section \ref{sec43}.


In addition, the drift term in \ref{sdeSigma} is equal to $\frac12$ the gradient of log volume of orbit $\mathcal O_{\lambda}$, as a parallel to Coulomb potential in Dyson Brownian motion.
\begin{theorem}\label{thm2}
    For $\lambda\in\Lambda$, the log volume of orbit $\mathcal O_{\lambda}$ is given by the following
    \begin{align}
        \log\mathrm{Vol}(\mathcal O_{\lambda})=&2\Phi=\sum_{k=1}^n\log\sinh{\sigma^k}+\sum_{1\leq k<l\leq n}\log|\cosh{\sigma^k}-\cosh{\sigma^l}|+c
    \end{align}
    so equation \ref{sdeSigma} could be written as a Langevin equation 
    \begin{align}
        \ud \sigma^k_t=\frac{\partial \Phi}{\partial \sigma^k}\ud t+\sqrt{\frac2\beta}\ud W^k_t
    \end{align}
\end{theorem}

Proof of theorem \ref{thm2} will be provided in section \ref{sec52}. We should give a remark here about metric $g_{\Lambda}$ on $\Lambda$: since $\Lambda$ is a quotient space of $\mathcal H$ over $G_{\ii I_n}$, we could define metric $g_{\Lambda}$ on $\Lambda$ using Riemannian submersion. The $\sigma$ coordinate is special for Riemannian manifold $(\Lambda,g_{\Lambda})$, as $g_{\Lambda}$ becomes Euclidean in this chart. A direct result is that the $k$-th component of $\mathrm{grad}\;\Phi$ is just equal to $\frac{\partial \Phi}{\partial \sigma^k}$. 

